Membership Inference on Word Embedding and Beyond

In the text processing context, most ML models are built on word embeddings. These embeddings are themselves trained on some datasets, potentially containing sensitive data. In some cases this training is done independently, in other cases, it occurs as part of training a larger, task-specific model. In either case, it is of interest to consider membership inference attacks based on the embedding layer as a way of understanding sensitive information leakage. But, somewhat surprisingly, membership inference attacks on word embeddings and their effect in other natural language processing (NLP) tasks that use these embeddings, have remained relatively unexplored. In this work, we show that word embeddings are vulnerable to black-box membership inference attacks under realistic assumptions. Furthermore, we show that this leakage persists through two other major NLP applications: classification and text-generation, even when the embedding layer is not exposed to the attacker. We show that our MI attack achieves high attack accuracy against a classifier model and an LSTM-based language model. Indeed, our attack is a cheaper membership inference attack on text-generative models, which does not require the knowledge of the target model or any expensive training of text-generative models as shadow models.

==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> generative.tex <==
\section{Embedding Attack on a Text-Generation Model}

In the previous section, we show an application of our embedding attack to a text-classification model. In this section, we extend our approach to attack a text-generation model. We focus on the next-word prediction task as the text-generation setting. This is a very popular setting in which language models have been deployed in practice to perform text auto-completion in emails and predictive keyboards \citep{swiftkey, gmailsc}. On the other hand, such models are extensively trained on personal data, e.g. users' emails, documents, chats etc., which may lead to privacy leakages as studies show in \citep{song19, secretsharer, carlini2020extracting, inan2021}.

\paragraph{Target model}
Similar to the setting in \citep{song19}, we use long short-term memory (LSTM) \citep{lstm} in our language model. LSTM is a special type of Recurrent Neural Networks (RNNs) that can capture the long-term dependency in the text sequence. In this network, the text sequence of tokens is first mapped to a sequence of embeddings. The embedding is then fed to the LSTM that learns a hidden representation for the context for predicting the next word. We use a two-layer LSTM model as the language model for the next-word prediction task. We set both the embedding dimension and LSTM hidden-representation size to 500 (gives around 50 million parameters). We use the Adam optimizer with the learning rate set to 1e-3 and batch size to 64. The performance of the model is presented in Table \ref{table:lm_perf}.

\begin{table}
\vskip 0.15in
\begin{subtable}[t]{0.45\textwidth}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}[t]{p{0.3\textwidth}p{0.22\textwidth}p{0.2\textwidth}}
\toprule
Model & Train perp & Test perp \\
\midrule
2-layer LSTM & 94.70 & 107.37 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Performance of target model. Perp stands for perplexity.}
\label{table:lm_perf}
\end{subtable}
\begin{subtable}[t]{0.5\textwidth}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}[t]{p{0.25\textwidth}p{0.18\textwidth}p{0.18\textwidth}p{0.18\textwidth}}
\toprule
Attack & Accuracy & Precision & Recall \\
\midrule
Our attack & 0.65 & 0.64 & 0.68 \\
Baseline 1 & 0.5 & 0.5 & 1.0 \\
Baseline 2 & 0.53 & 1.0 & 0.06 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Attack results of Section \ref{sec:mia_wout_threshold}. Baseline 1 is applying Algorithm \ref{alg:mia_wout_threshold} for \textbf{all word pairs} in a user's data. Baseline 2 is applying Algorithm \ref{alg:mia_wout_threshold} for all word pairs except the ones that can be found in a public dictionary (GloVe).}
\label{table:mia_wout_threshold}
\end{subtable}
\vskip -0.1in
\end{table}

\paragraph{Dataset} We use the Avocado dataset~\citep{avocado2015} in our experiments. We fix the vocabulary to the most frequent 40,000 tokens in the training corpus. Following the setting in \citep{song19}, we train the word-prediction model on the data of 50 randomly selected users and keep a different set of 50 randomly selected users as the test data. This roughly amounts to the half of the users in the data and the other half is utilized for the shadow data.

Recent work has shown both successful extraction of training data \citep{snapshotattack, carlini2020extracting, inan2021} and membership inference \citep{song19} in language models. The membership inference attack we describe in this section is different in the sense that our method only uses the top-1 predictions of the model, i.e. our attack is label-only, which is a strong and realistic attack setting that has been explored recently in visual domain as well \citep{choo2020labelonly, li2021membership}. We next describe two attack methods; one that works trivially without even any threshold selection hence being operationally/computationally efficient, second that requires threshold selection but achieving impressive precision-recall performance.  

\subsection{Label-only membership inference without threshold selection}
\label{sec:mia_wout_threshold}
The attack works as follows. For each user in the target dataset, we apply the attack described in Section \ref{sec:embed_attack} using the shadow dataset, which generates a list of word pairs $(w_i, w_{i+1})$. Let us denote this list as $\mathcal{W}$. The attack operates on each pair in $\mathcal{W}$ in a simple way by querying the model with $w_i$ and checking if the top prediction returned by the model is $w_{i+1}$. If there exists a pair of words in $\mathcal{W}$ satisfying this condition, the corresponding user is predicted as member. Otherwise, the user is predicted as non-member. The attack is described in Algorithm \ref{alg:mia_wout_threshold}.

\begin{algorithm}
   \caption{Label-only membership inference attack described in Section \ref{sec:mia_wout_threshold}.}
   \label{alg:mia_wout_threshold}
\begin{algorithmic}
   \STATE {\bfseries Input:} A language model $LM(\cdot)$, the user data $\mathcal{D}$, and the shadow data $\mathcal{S}$
   \STATE {\bfseries Output:} The membership prediction
   \STATE Obtain a list of word pairs $\mathcal{W}$ from embedding attack in Section \ref{sec:embed_attack} given $\mathcal{D}$ and $\mathcal{S}$
   \FOR{$(w_i, w_{i+1})$ {\bfseries in} $\mathcal{W}$}
   \STATE Query the model with $w_i$ and obtain the next-word prediction $p$
   \IF{$p = w_{i+1}$}
   \RETURN ``Member"
   \ENDIF
   \ENDFOR
   \RETURN ``Non-member"
\end{algorithmic}
\end{algorithm}

We note that for a member prediction, it is sufficient to have at least one pair of words satisfying the described condition. Therefore, a well-curated list of word pairs should be generated so that the condition is not satisfied for any of the word pairs for a non-member and it is satisfied for at least one pair for a member. The approach described in Section \ref{sec:embed_attack} is effective in the sense that it can generate such well-crafted list of word pairs for each user. The results are presented in Table \ref{table:mia_wout_threshold}. We point out that with label-only access and not training any shadow models, our attack performs impressively. There is no attack in such a setting to the best of our knowledge. For a baseline, we apply the attack in Algorithm \ref{alg:mia_wout_threshold} using all word pairs in a user's dataset. Naturally, this results in all-member prediction since each user has at least one word pair satisfying the required condition. We further removed the common words by excluding the word pairs if they are present in a public dictionary (we use GloVe public dictionary \citep{pennington2014glove}). Interestingly, the attack only predicts 3 users as members, however, indeed they are members. The results in Table \ref{table:mia_wout_threshold} show that our approach indeed generates a well-curated list of word pairs that provides good signal for membership inference.

We note that our attack has a computational advantage because it only requires training word2vec embeddings. It does not even need a threshold selection for membership prediction. In the next section, we will describe an attack method that does require threshold selection, but it achieves favorable precision-recall trade-off.

\subsection{Label-only threshold-based membership inference}
\label{sec:mia_w_threshold}
We extend the attack described in Section \ref{sec:mia_wout_threshold} to a threshold-based attack as follows. We similarly use the attack described in Section \ref{sec:embed_attack} to obtain a list of word pairs $\mathcal{W}$. We next calculate the average number of word pairs $(w_i , w_{i+1})$ where querying the model with $w_i$ yields the next-word prediction as $w_{i+1}$. For a threshold value $t$, a user is predicted member if the average number of word pairs satisfying the required condition is above $t$ and non-member otherwise. The attack is described in Algorithm \ref{alg:mia_w_threshold}.

\begin{algorithm}
   \caption{Label-only membership inference attack described in Section \ref{sec:mia_w_threshold}.}
   \label{alg:mia_w_threshold}
\begin{algorithmic}
   \STATE {\bfseries Input:} A language model $LM(\cdot)$, the user data $\mathcal{D}$, the shadow data $\mathcal{S}$, and a threshold value $t$
   \STATE {\bfseries Output:} The membership prediction
   \STATE Obtain a list of word pairs $\mathcal{W}$ from embedding attack in Section \ref{sec:embed_attack} given $\mathcal{D}$ and $\mathcal{S}$
   \STATE Set $count = 0$ 
   \FOR{$(w_i, w_{i+1})$ {\bfseries in} $\mathcal{W}$}
   \STATE Query the model with $w_i$ and obtain the next-word prediction $p$
   \IF{$p = w_{i+1}$}
   \STATE $count = count + 1$
   \ENDIF
   \ENDFOR
   \STATE Set $average = count/|\mathcal{W}|$
   \RETURN ``Member" if $average > t$ else ``Non-member"
\end{algorithmic}
\end{algorithm}



==> pending_experiments.tex <==
1. Selecting threshold based on shadow language data
	1. Shadow data from Avocado to begin with
2. Enron data for word2vec data
3. Aligning user/tenant
4. Try to do some trivial experiment for sanity check?
	1. Try word pairs not in the vocab
5.Try 0-1 threshold
6.Try best threshold both for all word pairs and word pairs not in public vocab
7. Repeat the threshold experiment with a different set of in and out users and plot the precision/recall. Just to make sure its the same across different users.
8. tenant level attack for generative model?[not top priority]
